UnMask: Adversarial Detection and Defense Through Robust Feature Alignment

Deep learning models are being integrated into a wide range of high-impact, security-critical systems, from self-driving cars to medical diagnosis. However, recent research has demonstrated that many of these deep learning architectures are vulnerable to adversarial attacks--highlighting the vital need for defensive techniques to detect and mitigate these attacks before they occur. To combat these adversarial attacks, we developed UnMask, an adversarial detection and defense framework based on robust feature alignment. The core idea behind UnMask is to protect these models by verifying that an image's predicted class ("bird") contains the expected robust features (e.g., beak, wings, eyes). For example, if an image is classified as "bird", but the extracted features are wheel, saddle and frame, the model may be under attack. UnMask detects such attacks and defends the model by rectifying the misclassification, re-classifying the image based on its robust features. Our extensive evaluation shows that UnMask (1) detects up to 96.75% of attacks, and (2) defends the model by correctly classifying up to 93% of adversarial images produced by the current strongest attack, Projected Gradient Descent, in the gray-box setting. UnMask provides significantly better protection than adversarial training across 8 attack vectors, averaging 31.18% higher accuracy. We open source the code repository and data with this paper: https://github.com/safreita1/unmask.

==> tables/dataset_conversion.tex <==
\begin{table}[t]
\scriptsize
% \setlength{\tabcolsep}{6pt}
\centering
 \begin{tabular}{p{1.5cm} p{6.5cm}} 
 \toprule
 \textbf{UnMask} & \textbf{PASCAL-Part} \\ [0.5ex] 
 \midrule
 Arm & Right upper arm, right lower arm, left upper arm, left lower arm \\ [0.5ex] 
 Beak & Beak \\ [0.5ex] 
 Body & Body \\ [0.5ex] 
 Cap & Cap \\ [0.5ex] 
 Coach back & Coach back (1-1) \\ [0.5ex] 
 Coach front & Coach front (1-9) \\ [0.5ex] 
 Coach left & Coach left (1-9) \\ [0.5ex] 
 Coach right & Coach right (1-8) \\ [0.5ex] 
 Coach top & Coach top (1-4) \\ [0.5ex] 
 Door & Door (1-4) \\ [0.5ex] 
 Engine & Engine (1-6) \\ [0.5ex] 
 Ear & Left ear, right ear \\ [0.5ex] 
 Eye & Left eye, right eye \\ [0.5ex] 
 Eyebrow & Left eyebrow, right eyebrow \\ [0.5ex] 
 Foot & Left foot, right foot \\ [0.5ex] 
 Front side & Front side \\ [0.5ex] 
 Hair & Hair \\ [0.5ex] 
 Hand & Left hand, right hand \\ [0.5ex] 
 Head & Head \\ [0.5ex] 
 Headlight & Left headlight (1-8) \\ [0.5ex] 
 Hoof &  Left back hoof, left front hoof, right back hoof, right front hoof \\ [0.5ex] 
 Horn & Left horn, right horn \\ [0.5ex] 
 Leg & Lower left leg, right front lower leg, right lower leg, left leg, left front leg, left front lower leg, right front upper leg, right back upper leg, left upper leg, left back upper leg, right leg, right back lower leg, right front leg, left back leg, right back leg, right upper leg, left back lower leg, left front upper leg \\ [0.5ex] 
 License plate & Back license plate, front license plate \\ [0.5ex] 
 Mirror & Left mirror, right mirror \\ [0.5ex] 
 Mouth & Mouth \\ [0.5ex] 
 Muzzle & Muzzle \\ [0.5ex] 
 Neck & Neck \\ [0.5ex] 
 Nose & Nose \\ [0.5ex] 
 Paw & Left back paw, left front paw, right back paw,  right front paw \\ [0.5ex] 
 Plant & Plant \\ [0.5ex] 
 Pot & Pot \\ [0.5ex] 
 Saddle & Saddle \\ [0.5ex] 
 Screen & Screen \\ [0.5ex] 
 Stern & Stern \\ [0.5ex] 
 Tail & Tail \\ [0.5ex] 
 Torso & Torso \\ [0.5ex] 
 Vehicle back & Vehicle back \\ [0.5ex] 
 Vehicle front & Vehicle front \\ [0.5ex] 
 Vehicle left & Vehicle left \\ [0.5ex] 
 Vehicle right & Vehicle right \\ [0.5ex] 
 Wheel & Wheel (1-8), back wheel, chainwheel, front wheel \\ [0.5ex] 
 Window & Window (1-20) \\ [0.5ex] 
 Wing & Left wing, right wing \\  [0.5ex] 
\bottomrule
\end{tabular}
\caption{Feature mapping from PASCAL-Part to the \dataset. We use the notation ``part (1-x)" to indicate that the PASCAL-Part dataset labeled the feature as `x' separate feature labels. We also note that the PASCAL-Part utilizes a more dense label notation, which we re-label in the table for ease of reading. For example, right front lower leg is abbreviated `rflleg' in PASCAL-Part. 
}
\label{feature_mapping}
\end{table}
